VIBE: Vector Index Benchmark for Embeddings

Approximate nearest neighbor (ANN) search is a performance-critical component of many machine learning pipelines, and rigorous benchmarking is essential for assessing the performance of vector indexes for ANN search. However, the datasets of existing benchmarks no longer represent modern ANN applications, creating a need for an up-to-date benchmark. To address this gap, we introduce Vector Index Benchmark for Embeddings (VIBE), an open-source framework for benchmarking ANN algorithms. VIBE provides a pipeline for generating benchmark datasets with dense embedding models representative of modern applications, including retrieval-augmented generation (RAG). To represent real-world workloads, we also include out-of-distribution (OOD) datasets where the queries and the corpus are drawn from different distributions. These include multimodal retrieval datasets and maximum inner product search (MIPS) datasets covering two recent use cases: approximate attention computation and reductions of multi-vector retrieval to single-vector MIPS. We use VIBE to conduct a comprehensive evaluation of 22 open-source vector-index implementations across 11 in-distribution and 8 out-of-distribution datasets. The benchmark is available at https://github.com/vector-index-bench/vibe

==> algtable.tex <==
\begin{NiceTabular}{@{}c@{}c@{}c@{}c@{}}
\Block[tikz={top color=gray!15}]{*-1}{}\textbf{graph-based} &
\Block[tikz={top color=blue!15}]{*-1}{}\textbf{clustering-based} &
\Block[tikz={top color=orange!15}]{*-1}{}\textbf{tree-based} &
\Block[tikz={top color=green!15}]{*-1}{}\textbf{hashing-based}\\
\href{https://github.com/zilliztech/pyglass}{GLASS} &
\href{https://github.com/google-research/google-research/tree/master/scann}{ScaNN}~\citeAlg{guo2020accelerating} &
\href{https://github.com/spotify/annoy}{ANNOY} &
\href{https://github.com/puffinn/puffinn}{PUFFINN}~\citeAlg{aumuller2019puffinn} \\
\href{https://github.com/lmcinnes/pynndescent}{PyNNDescent}~\citeAlg{wei2021pynndescent} &
\href{https://github.com/facebookresearch/faiss}{IVF}~\citeAlg{jegou2011product} &
\href{https://github.com/vioshyvo/mrpt}{MRPT}~\citeAlg{hyvonen2016fast} &
\href{https://github.com/NinhPham/FalconnPP}{\underline{FALCONN++}}~\citeAlg{pham2022falconn++} \\
\href{https://github.com/BlaiseMuhirwa/flatnav}{\underline{FlatNav}}~\citeAlg{munyampirwa2024down} &
\href{https://github.com/facebookresearch/faiss}{IVF-PQ}~\citeAlg{jegou2011product} &
\href{https://github.com/ejaasaari/mlann}{\underline{MLANN}}~\citeAlg{hyvonen2022multilabel} &
 \\
\href{https://github.com/matchyc/RoarGraph}{\underline{RoarGraph}}~\citeAlg{chen2024roargraph} &
\href{https://github.com/ejaasaari/lorann}{\underline{LoRANN}}~\citeAlg{jaasaari2024lorann} &
 &
 \\
\href{https://github.com/intel/ScalableVectorSearch}{\underline{LeanVec}}~\citeAlg{tepper2024leanvec} &
 &
 &
 \\
\href{https://github.com/intel/ScalableVectorSearch}{\underline{LVQ}}~\citeAlg{aguerrebere2023similarity} &
 &
 &
 \\
\href{https://github.com/gouyt13/SymphonyQG}{\underline{SymphonyQG}}~\citeAlg{gou2025symphonyqg} &
 &
 &
 \\
\end{NiceTabular}


==> algtable2.tex <==
\begin{NiceTabular}{ccccc}
\toprule
\multicolumn{2}{@{\hskip 24pt}c@{\hskip 24pt}}{\Block[fill=light_blue]{*-2}{}\textbf{Graphs}} &
\multicolumn{1}{@{\hskip 24pt}c@{\hskip 24pt}}{\Block[fill=light_purple]{*-1}{}\textbf{Trees}} &
\multicolumn{1}{@{\hskip 24pt}c@{\hskip 24pt}}{\Block[fill=light_green]{*-1}{}\textbf{Clustering}} &
\multicolumn{1}{@{\hskip 24pt}c@{\hskip 24pt}}{\Block[fill=light_orange]{*-1}{}\textbf{Hashing}}\\
\midrule
\href{https://github.com/zilliztech/pyglass}{Glass} &
\href{https://github.com/lmcinnes/pynndescent}{PyNNDescent} &
\href{https://github.com/spotify/annoy}{ANNOY} &
\href{https://github.com/facebookresearch/faiss}{IVF} &
\href{https://github.com/puffinn/puffinn}{PUFFINN} \\
\href{https://github.com/facebookresearch/faiss}{NSG} &
\href{https://github.com/nmslib/hnswlib}{HNSW} &
\href{https://github.com/vioshyvo/mrpt}{MRPT} &
\href{https://github.com/facebookresearch/faiss}{IVF-PQ} &
\href{https://github.com/NinhPham/FalconnPP}{FALCONN++${}^*$} \\
\href{https://github.com/NGT-labs/NGT/}{NGT-QG} &
\href{https://github.com/VectorDB-NTU/RaBitQ-Library}{HNSW-RaBitQ${}^*$} &
\href{https://github.com/ejaasaari/mlann}{MLANN${}^*$} &
\href{https://github.com/VectorDB-NTU/RaBitQ-Library}{IVF-RaBitQ${}^*$} &
 \\
\href{https://github.com/microsoft/DiskANN}{Vamana} &
\href{https://github.com/BlaiseMuhirwa/flatnav}{FlatNav${}^*$} &
 &
\href{https://github.com/google-research/google-research/tree/master/scann}{ScaNN} &
 \\
\href{https://github.com/intel/ScalableVectorSearch}{LVQ${}^*$} &
\href{https://github.com/intel/ScalableVectorSearch}{LeanVec${}^*$} &
 &
\href{https://github.com/ejaasaari/lorann}{LoRANN${}^*$} &
 \\
\href{https://github.com/matchyc/RoarGraph}{RoarGraph${}^*$} &
\href{https://github.com/gouyt13/SymphonyQG}{SymphonyQG${}^*$} &
 &
 &
 \\
\bottomrule
\end{NiceTabular}

==> algtable_sup.tex <==
\begin{NiceTabular}{lll}
\toprule
Method & Reference & Version\\\midrule
\rowcolor{light_purple} \href{https://github.com/spotify/annoy}{ANNOY} & \cite{annoy} & 1.17.3\\
\rowcolor{light_orange} \href{https://github.com/NinhPham/FalconnPP}{FALCONN++} & \cite{pham2022falconn++}& git+5fd3f17\\
\rowcolor{light_blue} \href{https://github.com/BlaiseMuhirwa/flatnav}{FlatNav} & \cite{munyampirwa2024down}& 0.1.2\\
\rowcolor{light_blue} \href{https://github.com/zilliztech/pyglass}{Glass} & \cite{PyGlass} & git+d2296ec\\
\rowcolor{light_blue} \href{https://github.com/nmslib/hnswlib}{HNSW} & \cite{malkov2018efficient}& 0.8.0\\
\rowcolor{light_blue} \href{https://github.com/VectorDB-NTU/RaBitQ-Library}{HNSW-RaBitQ} & \cite{gao2024rabitq,gao2025practical,gao2025rabitq} & git+5ea4df0\\
\rowcolor{light_green} \href{https://github.com/facebookresearch/faiss}{IVF} & \cite{jegou2011product,douze2024faiss}& 1.14.3\\
\rowcolor{light_green} \href{https://github.com/facebookresearch/faiss}{IVF-PQ} & \cite{jegou2011product,douze2024faiss}& 1.14.3\\
\rowcolor{light_green} \href{https://github.com/VectorDB-NTU/RaBitQ-Library}{IVF-RaBitQ} & \cite{gao2024rabitq,gao2025rabitq,gao2025practical} & git+5ea4df0\\
\rowcolor{light_blue} \href{https://github.com/intel/ScalableVectorSearch}{LVQ} & \cite{aguerrebere2023similarity}& 0.4.0\\
\rowcolor{light_blue} \href{https://github.com/intel/ScalableVectorSearch}{LeanVec} & \cite{tepper2024leanvec}& 0.4.0\\
\rowcolor{light_green} \href{https://github.com/ejaasaari/lorann}{LoRANN} & \cite{jaasaari2024lorann}& 0.4.5\\
\rowcolor{light_purple} \href{https://github.com/ejaasaari/mlann}{MLANN} & \cite{hyvonen2022multilabel}& git+ba141b4\\
\rowcolor{light_purple} \href{https://github.com/vioshyvo/mrpt}{MRPT} & \cite{hyvonen2016fast,jaasaari2019efficient}& 2.0.4\\
\rowcolor{light_blue} \href{https://github.com/NGT-labs/NGT/}{NGT-ONNG} & \cite{iwasaki2018optimization,ngt} & 2.7.4\\
\rowcolor{light_blue} \href{https://github.com/NGT-labs/NGT/}{NGT-QG} & \cite{ngt} & 2.7.4\\
\rowcolor{light_blue} \href{https://github.com/facebookresearch/faiss}{NSG} & \cite{fu2017nsg,douze2024faiss}& 1.14.3\\
\rowcolor{light_orange} \href{https://github.com/puffinn/puffinn}{PUFFINN} & \cite{aumuller2019puffinn}& git+fd86b0d\\
\rowcolor{light_blue} \href{https://github.com/lmcinnes/pynndescent}{PyNNDescent} & \cite{wei2021pynndescent,pynndescent}& 0.6.0\\
\rowcolor{light_blue} \href{https://github.com/matchyc/RoarGraph}{RoarGraph} & \cite{chen2024roargraph}& git+f2b49b6\\
\rowcolor{light_green} \href{https://github.com/google-research/google-research/tree/master/scann}{ScaNN} & \cite{guo2020accelerating}& 1.4.2\\
\rowcolor{light_blue} \href{https://github.com/gouyt13/SymphonyQG}{SymphonyQG} & \cite{gou2025symphonyqg}& git+32a0019\\
\rowcolor{light_blue} \href{https://github.com/microsoft/DiskANN}{Vamana} & \cite{jayaram2019diskann}& 0.7.0\\
\bottomrule
\end{NiceTabular}


==> tables/algorithm-implementations.tex <==
\begin{table}[!htbp]
\centering
\caption{Details of the algorithm implementations included in the benchmark.}
\label{tab:impdetails}
\input{algtable_sup.tex}
\vspace*{6pt}
\end{table}


==> tables/algorithms-summary.tex <==
\begin{table*}[!t]
\centering
\caption{Summary of the evaluated algorithms. `*' marks implementations that have not been included in earlier benchmarks. See Table~\ref{tab:impdetails} in Appendix~\ref{app:impdetails} for citations and implementation details.}
\label{tab:algorithms}
\input{algtable2.tex}
\vspace*{2pt}
\end{table*}


==> tables/data-sources.tex <==
\begin{table*}[!htbp]
\begin{threeparttable}
\begin{center}
\caption{Data sources used to produce the \textsc{VIBE} embedding datasets.}
\label{tab:datasources}
    \setlength{\tabcolsep}{0pt}
    \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}llrrl@{}}
        \toprule
        Name & Type & $n$ & Reference & Citation \\
        \midrule
        AGNews & Text & 770 382 & \tnote{1} & N/A \\
        arXiv abstracts & Text & 1 345 643 & \tnote{2} & N/A \\
        CQADupStack & Text & 457 149 & \tnote{3} & \cite{hoogeveen2015cqadupstack} \\
        DPR & Text & 20 970 760 & \tnote{4} & \cite{karpukhin2020dense} \\
        GooAQ & Text & 1 476 024 & \tnote{5} & \cite{khashabi2021gooaq} \\
        HotpotQA & Text & 5 233 329 & \tnote{6} & \cite{yang2018hotpotqa} \\
        ImageNet & Image & 1 281 167 & \tnote{7} & \cite{deng2009imagenet} \\
        ImageNet-Captions & Text & 316 648 & \tnote{8} & \cite{fang2022data} \\
        iNaturalist Mini & Image & 500 000 & \tnote{9} & \cite{vanhorn2021benchmarking} \\
        Landmark & Image & 761 757 & \tnote{10} & \cite{weyand2020google} \\
        MS MARCO & Text & 8 841 823 & \tnote{11} & \cite{bajaj2016ms} \\
        Yahoo Answers & Text & 678 305 & \tnote{12} & N/A \\
        \bottomrule
    \end{tabular*}
\begin{tablenotes}
    \item [1] \url{http://groups.di.unipi.it/~gulli/AG_corpus_of_news_articles.html}
    \item [2] \url{https://www.kaggle.com/datasets/Cornell-University/arxiv}
    \item [3] \url{http://nlp.cis.unimelb.edu.au/resources/cqadupstack/}
    \item [4] \url{https://github.com/facebookresearch/DPR}
    \item [5] \url{https://github.com/allenai/gooaq}
    \item [6] \url{https://hotpotqa.github.io/}
    \item [7] \url{https://www.image-net.org/}
    \item [8] \url{https://github.com/mlfoundations/imagenet-captions}
    \item [9] \url{https://github.com/visipedia/inat_comp/tree/master/2021}
    \item [10] \url{https://github.com/cvdfoundation/google-landmark}
    \item [11] \url{https://microsoft.github.io/msmarco/}
    \item [12] \url{https://www.kaggle.com/datasets/soumikrakshit/yahoo-answers-dataset}
\end{tablenotes}
\end{center}
\end{threeparttable}
\end{table*}


==> tables/embedding-models.tex <==
\begin{table*}[!htbp]
    \centering
    \caption{Embedding models used to produce the \textsc{VIBE} datasets. The license for each embedding applies to the model; none of the models claim rights over their outputs.}
    \label{tab:embeddings}
    \setlength{\tabcolsep}{0pt}
    \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lllll@{}}
        \toprule
        Name & Model & Citation & License \\
        \midrule
        ALIGN & \href{https://huggingface.co/kakaobrain/align-base}{align-base} & \cite{jia2021scaling} & Custom \\
        CLIP & \href{https://huggingface.co/openai/clip-vit-base-patch32}{clip-vit-base-patch32} & \cite{radford2021learning} & MIT \\
        DINO & \href{https://huggingface.co/timm/vit_base_patch16_224.dino}{vit\_base\_patch16\_224.dino} & \cite{caron2021emerging} & Apache 2.0 \\
        DistilRoBERTa & \href{https://huggingface.co/sentence-transformers/all-distilroberta-v1}{all-distilroberta-v1}{} & \cite{sanh2019distilbert} & Apache 2.0 \\
        Harrier & \href{https://huggingface.co/microsoft/harrier-oss-v1-270m}{harrier-oss-v1-270m} & - & MIT \\
        Jina & \href{https://huggingface.co/jinaai/jina-embeddings-v5-text-nano}{jina-embeddings-v5-text-nano} & \cite{akram2026jina} & CC-BY-NC-4.0 \\
        MiniLM & \href{https://huggingface.co/sentence-transformers/all-MiniLM-L6-v2}{all-MiniLM-L6-v2} & \cite{wang2020minilm} & Apache 2.0 \\
        MXBAI & \href{https://huggingface.co/mixedbread-ai/mxbai-embed-large-v1}{mxbai-embed-large-v1} & \cite{emb2024mxbai} & Apache 2.0 \\
        Nomic Text & \href{https://huggingface.co/nomic-ai/nomic-embed-text-v1.5}{nomic-embed-text-v1.5} & \cite{nussbaum2025nomic} & Apache 2.0 \\
        Nomic Vision & \href{https://huggingface.co/nomic-ai/nomic-embed-vision-v1.5}{nomic-embed-vision-v1.5} & \cite{nussbaum2024nomic} & Apache 2.0 \\
        Qwen & \href{https://huggingface.co/Qwen/Qwen3-Embedding-0.6B}{Qwen3-Embedding-0.6B} & \cite{qwen3embedding} & Apache 2.0 \\
        ResNet & \href{https://docs.pytorch.org/vision/main/models/generated/torchvision.models.resnet50.html}{resnet50} & \cite{he2016deep} & BSD 3 \\
        \bottomrule
    \end{tabular*}
\end{table*}


==> tables/gpu-algorithm-implementations.tex <==
\begin{table}[!htbp]
\centering
\caption{Details of the GPU algorithm implementations included in the benchmark.}
\label{tab:gpu-algorithms}
\begin{NiceTabular}{lll}
\toprule
Method & Reference & Version\\\midrule
\rowcolor{light_blue} \href{https://github.com/rapidsai/cuvs}{CAGRA (cuVS)} & \cite{ootomo2024cagra,cuvs} & 26.04.00\\
\rowcolor{light_blue} \href{https://github.com/cgtuebingen/ggnn}{GGNN} & \cite{groh2022ggnn} & 0.9\\
\rowcolor{light_green} \href{https://github.com/rapidsai/cuvs}{IVF-PQ (cuVS)} & \cite{cuvs} & 26.04.00\\
\rowcolor{light_green} \href{https://github.com/rapidsai/cuvs}{IVF (cuVS)} & \cite{cuvs} & 26.04.00\\
\rowcolor{light_green} \href{https://github.com/facebookresearch/faiss}{IVF (Faiss)} & \cite{johnson2019billion,douze2024faiss} & 1.14.3\\
\bottomrule
\end{NiceTabular}
\vspace*{6pt}
\end{table}


==> tables/hypervolume.tex <==
\begin{table*}[ht!]
\centering
\caption{Normalized hypervolume of recall--throughput curves over average recall $[0.9, 1]$. The final column gives mean $\pm$ standard deviation across datasets with rows sorted by decreasing mean. Colors denote \protect\ulc{clustering}{color_green}, \protect\ulc{tree}{color_purple}, \protect\ulc{hashing}{color_orange}, and \protect\ulc{graph}{color_blue} methods.}
\label{table:hypervolume}
\newcommand{\hvsummarystat}[2]{$#1$\,{\fontsize{7}{8}\selectfont\scalebox{0.72}{$\pm$}$#2$}}
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{0.95}
\begin{NiceTabular}{>{\small}l r r r r r r r r r r | >{\footnotesize}r }
\toprule
{\small algorithm} &
\rotatebox{90}{\small agnews-mxbai} &
\rotatebox{90}{\small arxiv-nomic} &
\rotatebox{90}{\small glove} &
\rotatebox{90}{\small gooaq-distilroberta} &
\rotatebox{90}{\small imagenet-clip} &
\rotatebox{90}{\small inaturalist-resnet} &
\rotatebox{90}{\small landmark-dino} &
\rotatebox{90}{\small landmark-nomic} &
\rotatebox{90}{\small msmarco-qwen} &
\rotatebox{90}{\small yahoo-minilm} &
\multicolumn{1}{c}{\rotatebox{90}{\small \shortstack{hypervolume\\(mean $\pm$ sd)}}} \\
\midrule
\rowcolor{light_blue} glass & 0.67 & 0.83 & 0.16 & 0.71 & 0.86 & 0.83 & 0.72 & 0.84 & 0.57 & 0.63 & \hvsummarystat{0.68}{0.20} \\
\rowcolor{light_blue} ngt-qg & 0.73 & 0.80 & 0.52 & 0.69 & 0.75 & 0.85 & 0.79 & 0.77 & 0.00 & 0.71 & \hvsummarystat{0.66}{0.24} \\
\rowcolor{light_blue} symphonyqg & 0.60 & 0.81 & 0.18 & 0.59 & 0.81 & 0.00 & 0.72 & 0.57 & 0.76 & 0.54 & \hvsummarystat{0.56}{0.26} \\
\rowcolor{light_blue} rabitq-hnsw & 0.35 & 0.42 & 0.09 & 0.30 & 0.42 & 0.67 & 0.36 & 0.49 & 0.38 & 0.27 & \hvsummarystat{0.38}{0.14} \\
\rowcolor{light_green} lorann & 0.25 & 0.33 & 0.06 & 0.22 & 0.61 & 0.50 & 0.47 & 0.63 & 0.07 & 0.25 & \hvsummarystat{0.34}{0.20} \\
\rowcolor{light_blue} vamana-leanvec(svs) & 0.34 & 0.35 & 0.06 & 0.32 & 0.30 & 0.48 & 0.32 & 0.37 & 0.37 & 0.25 & \hvsummarystat{0.32}{0.10} \\
\rowcolor{light_blue} hnswlib & 0.26 & 0.33 & 0.13 & 0.30 & 0.42 & 0.38 & 0.28 & 0.45 & 0.25 & 0.24 & \hvsummarystat{0.30}{0.09} \\
\rowcolor{light_blue} flatnav & 0.23 & 0.29 & 0.10 & 0.30 & 0.43 & 0.39 & 0.26 & 0.45 & 0.23 & 0.22 & \hvsummarystat{0.29}{0.10} \\
\rowcolor{light_blue} pynndescent & 0.24 & 0.31 & 0.14 & 0.35 & 0.45 & 0.09 & 0.30 & 0.41 & 0.20 & 0.26 & \hvsummarystat{0.27}{0.11} \\
\rowcolor{light_blue} vamana-lvq(svs) & 0.26 & 0.30 & 0.09 & 0.29 & 0.28 & 0.00 & 0.27 & 0.28 & 0.35 & 0.23 & \hvsummarystat{0.23}{0.10} \\
\rowcolor{light_green} scann & 0.15 & 0.21 & 0.26 & 0.11 & 0.35 & 0.33 & 0.32 & 0.29 & 0.04 & 0.22 & \hvsummarystat{0.23}{0.10} \\
\rowcolor{light_blue} nsg(faiss) & 0.20 & 0.23 & 0.00 & 0.22 & 0.30 & 0.47 & 0.20 & 0.31 & 0.20 & 0.15 & \hvsummarystat{0.23}{0.11} \\
\rowcolor{light_green} ivfpqfs(faiss) & 0.10 & 0.22 & 0.32 & 0.14 & 0.30 & 0.28 & 0.30 & 0.29 & 0.06 & 0.23 & \hvsummarystat{0.22}{0.09} \\
\rowcolor{light_green} rabitq-ivf & 0.15 & 0.18 & 0.13 & 0.10 & 0.25 & 0.32 & 0.24 & 0.30 & 0.07 & 0.23 & \hvsummarystat{0.20}{0.08} \\
\rowcolor{light_blue} vamana(diskann) & 0.14 & 0.15 & 0.13 & 0.14 & 0.21 & 0.20 & 0.15 & 0.16 & 0.16 & 0.14 & \hvsummarystat{0.16}{0.03} \\
\rowcolor{light_green} ivf(faiss) & 0.03 & 0.04 & 0.05 & 0.02 & 0.09 & 0.06 & 0.06 & 0.09 & 0.00 & 0.05 & \hvsummarystat{0.05}{0.03} \\
\rowcolor{light_purple} mrpt & 0.03 & 0.03 & 0.03 & 0.03 & 0.03 & 0.03 & 0.03 & 0.07 & 0.00 & 0.04 & \hvsummarystat{0.03}{0.02} \\
\rowcolor{light_purple} annoy & 0.02 & 0.03 & 0.02 & 0.01 & 0.06 & 0.04 & 0.03 & 0.05 & 0.01 & 0.02 & \hvsummarystat{0.03}{0.02} \\
\rowcolor{light_orange} falconnpp & 0.00 & 0.01 & 0.05 & 0.02 & 0.02 & 0.04 & 0.02 & 0.01 & 0.01 & 0.03 & \hvsummarystat{0.02}{0.01} \\
\rowcolor{light_orange} puffinn & 0.00 & 0.00 & 0.02 & 0.02 & 0.01 & 0.03 & 0.02 & 0.01 & 0.00 & 0.02 & \hvsummarystat{0.01}{0.01} \\
\bottomrule
\end{NiceTabular}
\end{table*}


==> tables/id-datasets.tex <==
\begin{table}[t]
    \centering
    \caption[]{\textsc{VIBE} in-distribution datasets. For references and details about the data sources and embedding models, see Appendix~\ref{sec:models-data-sources}. Embeddings with measure ``any'' are normalized to unit norm, and each algorithm can choose an appropriate measure. Text datasets are highlighted in \ulc{green}{color_green} and image datasets are highlighted in \ulc{purple}{color_purple}. }
    \label{tab:id-datasets}
    \begin{tabular}{llrrl}
        \toprule
        Data Source & Model & $m$ & $d$ & Measure \\
        \midrule
        \rowcolor{light_green} AGNews & MXBAI & 769 382 & 1024 & Euclidean \\
        \rowcolor{light_green}arXiv abstracts & Nomic Text & 1 344 643 & 768 & any \\
        \rowcolor{light_green}DPR & Jina & 20 969 760 & 768 & any \\
        \rowcolor{light_green}GooAQ & DistilRoBERTa & 1 475 024 & 768 & any \\
        \rowcolor{light_purple}ImageNet & CLIP & 1 281 167 & 512 & any \\
        \rowcolor{light_purple}iNaturalist & ResNet & 499 000 & 2048 & cosine \\
        \rowcolor{light_purple}Landmark & DINO & 760 757 & 768 & cosine \\
        \rowcolor{light_purple}Landmark & Nomic Vision & 760 757 & 768 & any \\
        \rowcolor{light_green}MS MARCO & Qwen & 8 840 823 & 1024 & any \\
        \rowcolor{light_green}Yahoo Answers & MiniLM & 677 305 & 384 & any \\
        \rowcolor{light_green}- & GloVe & 1 192 514 & 200 & cosine \\
        \bottomrule
    \end{tabular}
\end{table}


==> tables/index-construction-times.tex <==
\begin{table*}[!htbp]
\centering
\caption{Index construction times (seconds) with throughput-optimized hyperparameters at $95\%$ average recall. The final column reports the mean $\pm$ standard deviation of construction time relative to the fastest construction time on each dataset. Algorithms are ordered by mean relative build time. \protect\ulc{Clustering}{color_green} methods are highlighted in green, \protect\ulc{tree}{color_purple} in purple, \protect\ulc{hashing}{color_orange} in orange, and \protect\ulc{graph}{color_blue} in blue.}
\label{table:construction}
\newcommand{\relbuildtime}[2]{$#1$\,{\fontsize{7}{8}\selectfont\scalebox{0.72}{$\pm$}$#2$}}
\setlength{\tabcolsep}{2.2pt}
\begin{NiceTabular}{>{\small}l r r r r r r r r r r !{\hspace{2pt}} | >{\footnotesize}r}
\toprule
\multicolumn{1}{l}{algorithm} &
\multicolumn{1}{c}{\rotatebox{90}{\small agnews-mxbai}} &
\multicolumn{1}{c}{\rotatebox{90}{\small arxiv-nomic}} &
\multicolumn{1}{c}{\rotatebox{90}{\small glove}} &
\multicolumn{1}{c}{\rotatebox{90}{\small gooaq-distilroberta}} &
\multicolumn{1}{c}{\rotatebox{90}{\small imagenet-clip}} &
\multicolumn{1}{c}{\rotatebox{90}{\small inaturalist-resnet}} &
\multicolumn{1}{c}{\rotatebox{90}{\small landmark-dino}} &
\multicolumn{1}{c}{\rotatebox{90}{\small landmark-nomic}} &
\multicolumn{1}{c}{\rotatebox{90}{\small msmarco-qwen}} &
\multicolumn{1}{c@{\hspace{3.8pt}}|}{\rotatebox{90}{\small yahoo-minilm}} &
\multicolumn{1}{c}{\rotatebox{90}{\footnotesize \shortstack{relative build time\\(mean $\pm$ sd)}}} \\
\midrule
\rowcolor{light_green} ivfpqfs(faiss) & 92 & 81 & 71 & 82 & 35 & 145 & 69 & 35 & 561 & 38 & \relbuildtime{1.4}{0.6} \\
\rowcolor{light_green} rabitq-ivf & 78 & 77 & 235 & 79 & 56 & 47 & 70 & 58 & 395 & 23 & \relbuildtime{1.4}{0.8} \\
\rowcolor{light_green} ivf(faiss) & 214 & 571 & 63 & 563 & 432 & 108 & 50 & 443 & 394 & 246 & \relbuildtime{5.8}{4.5} \\
\rowcolor{light_green} scann & 689 & 761 & 412 & 764 & 479 & 1004 & 468 & 248 & 5497 & 241 & \relbuildtime{11.1}{4.1} \\
\rowcolor{light_blue} glass & 987 & 929 & - & 1045 & 658 & 535 & 797 & 375 & 11674 & 562 & \relbuildtime{16.5}{6.1} \\
\rowcolor{light_blue} pynndescent & 327 & 427 & 2524 & 965 & 288 & 2136 & 551 & 230 & 11404 & 384 & \relbuildtime{17.9}{14.2} \\
\rowcolor{light_blue} vamana-leanvec(svs) & 1052 & 1499 & - & 1698 & 912 & 501 & 596 & 427 & 10369 & 774 & \relbuildtime{19.4}{7.5} \\
\rowcolor{light_purple} mrpt & 1263 & 1872 & 870 & 1966 & 1424 & 1037 & 1023 & 988 & - & 623 & \relbuildtime{24.1}{7.3} \\
\rowcolor{light_orange} puffinn & - & 2106 & 676 & 2363 & 1147 & - & 1258 & 1231 & - & 689 & \relbuildtime{27.2}{7.3} \\
\rowcolor{light_blue} vamana-lvq(svs) & 1823 & 2219 & - & 2323 & 1070 & - & 1133 & 1017 & 14797 & 832 & \relbuildtime{29.6}{4.8} \\
\rowcolor{light_purple} annoy & 446 & 2797 & 2125 & 3072 & 487 & 2197 & 2341 & 354 & 22873 & 948 & \relbuildtime{33.1}{16.6} \\
\rowcolor{light_green} lorann & 1149 & 1656 & - & 3526 & 2706 & 1086 & 1045 & 1773 & 19055 & 1539 & \relbuildtime{40.7}{20.7} \\
\rowcolor{light_blue} flatnav & 1585 & 3021 & 5509 & 3231 & 1362 & 1890 & 2075 & 909 & 16878 & 1542 & \relbuildtime{44.3}{18.3} \\
\rowcolor{light_blue} nsg(faiss) & 2256 & 2863 & - & 2796 & 2485 & 1626 & 2069 & 1801 & 20204 & 1465 & \relbuildtime{46.0}{13.3} \\
\rowcolor{light_blue} symphonyqg & 2207 & 3152 & - & 4085 & 2013 & - & 1760 & 1589 & 23779 & 1437 & \relbuildtime{47.6}{11.4} \\
\rowcolor{light_orange} falconnpp & - & 2843 & 1906 & 1573 & 3152 & 1762 & 927 & 2994 & 28190 & 1343 & \relbuildtime{49.6}{25.7} \\
\rowcolor{light_blue} hnswlib & 2211 & 3090 & 7591 & 3521 & 1627 & 2069 & 2005 & 863 & 30935 & 1165 & \relbuildtime{51.8}{26.8} \\
\rowcolor{light_blue} vamana(diskann) & 2393 & 4407 & 4237 & 3597 & 2378 & 1644 & 1546 & 2178 & 31148 & 1205 & \relbuildtime{52.7}{16.0} \\
\rowcolor{light_blue} rabitq-hnsw & 4610 & 4592 & 11013 & 7820 & 3138 & 3350 & 3375 & 2218 & 33884 & 2814 & \relbuildtime{89.1}{34.2} \\
\rowcolor{light_blue} ngt-qg & 14735 & 7352 & 40140 & 12047 & 3898 & 7977 & 5188 & 3486 & - & 7665 & \relbuildtime{209.7}{166.3} \\
\bottomrule
\end{NiceTabular}
\end{table*}


==> tables/ood-datasets.tex <==
\begin{table}[t]
    \centering
    \caption{\textsc{VIBE} out-of-distribution datasets. For details about the data sources and embedding models, see Appendix~\ref{sec:models-data-sources}. Embeddings with dissimilarity measure ``any'' are normalized to unit norm, and each algorithm can choose an appropriate measure. The two CQADupStack reductions and the \texttt{llama} and \texttt{yi} datasets are MIPS workloads and use (negative) inner product. Here $m$ = number of corpus points, $m_\text{learn}$ = number of query distribution samples, $d$ = embedding dimension.}
    \label{tab:ood-datasets}
    \begin{tabular}{lllrrrl}
        \toprule
        Data Source & Model & Type & $m$ ($\downarrow$) & $m_{\mathrm{learn}}$ & $d$ & Measure \\
        \midrule
        HotpotQA & Harrier & Text & 5 233 329 & 96 845 & 640 & any \\
        ImageNet & ALIGN & Text-To-Image & 1 281 167 & 315 648 & 640 & any \\
        LAION & CLIP & Text-To-Image & 1 000 448 & 999 448 & 512 & any \\
        Yandex & SE-ResNeXt & Text-To-Image & 999 000 & 999 000 & 200 & cosine \\
        CQADupStack & MUVERA & Multi-vector & 457 149 & 1 331 947 & 5120 & IP \\
        CQADupStack & LEMUR & Multi-vector & 457 149 & 1 331 947 & 2048 & IP \\
        Llama-3-8B & - & Attention & 256 921 & 255 921 & 128 & IP \\
        Yi-6B-200K & - & Attention & 187 843 & 186 843 & 128 & IP \\
        \bottomrule
    \end{tabular}
\end{table}

